Adapting Language Models for Zero-shot Learning by Meta-tuning on Dataset and Prompt Collections

Large pre-trained language models (LMs) such as GPT-3 have acquired a surprising ability to perform zero-shot learning. For example, to classify sentiment without any training examples, we can "prompt" the LM with the review and the label description "Does the user like this movie?", and ask whether the next word is "yes" or "no". However, the next word prediction training objective is still misaligned with the target zero-shot learning objective. To address this weakness, we propose meta-tuning, which directly optimizes the zero-shot learning objective by fine-tuning pre-trained language models on a collection of datasets. We focus on classification tasks, and construct the meta-dataset by aggregating 43 existing datasets and annotating 441 label descriptions in a question-answering (QA) format. When evaluated on unseen tasks, meta-tuned models outperform a same-sized QA model and the previous SOTA zero-shot learning system based on natural language inference. Additionally, increasing parameter count from 220M to 770M improves AUC-ROC scores by 6.3%, and we forecast that even larger models would perform better. Therefore, measuring zero-shot learning performance on language models out-of-the-box might underestimate their true potential, and community-wide efforts on aggregating datasets and unifying their formats can help build models that answer prompts better.

==> old_results.tex <==
\section{Results} \label{sec:results}
We evaluate a model by computing the AUC-ROC score for each label descriptions (Figure \ref{fig:data-collection}), or calculating its performance on the three benchmark datasets provided by \citet{yin-etal-2019-benchmarking}.
Both evaluation strategies lead to the same two conclusions: 
\begin{itemize}
    \item Meta(770M) outperforms QA(770M). Further specialization in ZSC is effective.
    \item Meta(770M) outperforms Meta(220M). Bigger models are better.
\end{itemize}

\subsection{Description-wise AUC-ROC} \label{sec:scatter}

\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/scatter.pdf}
    \caption{Each dot represents a label description, its x-value represents the AUC-ROC score of one model, and its y-value represents that of the other model.
    The left figure compares QA (x) vs. Meta-tuning (y) with the same model size (770M), and the right figure compares Meta-tuning on different model sizes: 220M (x) vs. 770M (y). 
    Since most dot is above the red line $y=x$ for both the left and the right figure, larger meta-tuned models are better. 
    }
    \label{fig:scatter}
\end{figure}
For each label description (question), we calculate the AUC-ROC score by treating the ``Yes" answer as the positive class. 
We do not evaluate F-score or accuracy, since they are very sensitive to the decision cutoff threshold, and usually additional calibration is needed \citet{Zhao2021Calibrate}.
We use a scatter plot to compare two models, where each dot represents a label description, its x-value represents the AUC-ROC score of one model, and its y-value represents that of the other model.

We generally do not try to aggregate a model's performances on different datasets into a single number and compare this number only.
The reasons are as follows: 1) it is unclear a priori how to aggregate AUC-ROC scores; for example, even if dataset A and dataset B are equally important, it is not clear whether scores (0.6, 0.9) or (0.75, 0.8) is better. 2) aggregate statistics remove lower-level information on the description-wise difference between AUC-ROC scores of the two models. 
We only resort to aggregate statistics when the conclusion is unclear based on visualizations. 


The results are in Figure \ref{fig:scatter}. 
Since most dots are above the red line, we conclude that, for most labels, larger/meta-tuned models are better.

\subsection{Benchmarking with \citet{yin-etal-2019-benchmarking}}
We compare our models on the zero shot classification datasets proposed by \citet{yin-etal-2019-benchmarking}, which consist of 3 multi-label classification datasets: emotion, situation, and topic classification. 
We use the exact same evaluation metrics and label resolution strategy when the model answers ``Yes" for multiple labels.

\begin{table}[]
    \centering
    \begin{tabular}{lccc}
        \hline
        Model & emotion & situation & topic \\
        \hline
        Prior(335M) & 25.2 & 38.0 & 52.1\\
        QA(770M) & 21.7 & 21.5 & 46.3 \\
        Meta(220M) & 26.2 & 33.8 & 51.4 \\
        Meta(770M) & \textbf{27.0} & \textbf{43.2} & \textbf{58.9} \\
        \hline
    \end{tabular}
    \caption{Evaluating on the 3 datasets from \citet{yin-etal-2019-benchmarking}: emotion, situation, and topic. The first two uses weighted F-score and the last uses accuracy as the evaluation metrics. ``Prior" means the best performing system from \citet{yin-etal-2019-benchmarking} for each dataset. We observe that meta-tuned larger models are better.
    }
    \label{tab:benchmarking}
\end{table}

The results can be seen in Table \ref{tab:benchmarking}. 
For reference, we also list the best performing system for each dataset from \citet{yin-etal-2019-benchmarking} (Prior), which uses a natural language inference system based on RoBERTA-large (355M parameters, \citet{liu2020roberta}), ensembles several different models, and uses other auxillary training objectives such as categorizing Wikipedia articles.
Similar to Section \ref{sec:scatter}, we find that larger/meta-tuned model are better for all 3 datasets.
Additionally, after controlling for the parameter count, our meta-tuned model (220 M) is comparable to the prior best system (335M).

\subsection{Robustness Checks}
We examine a series of additional results to ensure that our conclusions are robust.

We visualized with the same opacity for each label description in Figure \ref{fig:scatter}, which implicitly assumes that each description is equally important for evaluation. 
To ensure that the improvement is not caused by the improvement of a small number of labels that have more annotated descriptions, or by the improvement on a dataset that has more distinct labels, Appendix \ref{appendix-sec:more-viz} performs the same visualization with opacities inverse to the number of descriptions for each label/dataset. 

To provide additional supporting evidence for our forecast that larger models are better, Appendix \ref{appendix-sec:t5-larger-better} compares Meta(60M) with Meta(220M) and finds that the later is much better.

Another concern is that our models are initialized with T5 \cite{raffel2019exploring}, which is trained on the open web and might have seen the datasets we gathered. 
We address this in Appendix \ref{appendix-sec:bert-larger-better} by showing that larger models are also better with BERT \citet{devlin-etal-2019-bert}, which is trained on Wikipedia and Book Corpus \cite{zhu2015aligning}.




